Schr\"{o}dinger PCA: On the Duality between Principal Component Analysis and Schr\"{o}dinger Equation

Principal component analysis (PCA) has achieved great success in unsupervised learning by identifying covariance correlations among features. If the data collection fails to capture the covariance information, PCA will not be able to discover meaningful modes. In particular, PCA will fail the spatial Gaussian Process (GP) model in the undersampling regime, i.e. the averaged distance of neighboring anchor points (spatial features) is greater than the correlation length of GP. Counterintuitively, by drawing the connection between PCA and Schr\"odinger equation, we can not only attack the undersampling challenge but also compute in an efficient and decoupled way with the proposed algorithm called Schr\"odinger PCA. Our algorithm only requires variances of features and estimated correlation length as input, constructs the corresponding Schr\"odinger equation, and solves it to obtain the energy eigenstates, which coincide with principal components. We will also establish the connection of our algorithm to the model reduction techniques in the partial differential equation (PDE) community, where the steady-state Schr\"odinger operator is identified as a second-order approximation to the covariance function. Numerical experiments are implemented to testify the validity and efficiency of the proposed algorithm, showing its potential for unsupervised learning tasks on general graphs and manifolds.

==> SchPCA (pre)/response.tex <==
1.. Of course, these approximations are valid for the major
components only and become useless when the eigenfunction of (4) change
significantly on the correlation length. 

Yes, that's our setting for the model reduction.

2.This loss of validity is also obvious and unavoidable for growing index i in (4).

Not necessarily. Our method is robust even if we extract more eigenmodes, as long as the scale of the eigenmode is large so that it varies little over the correlation length.

3. Of course, a general second order elliptic equation
can be called “the Schrödinger equation”, and this analogy can help to somebody
but, at the same time, this is an elastic membrane equation, and there are many
other physically inspired analogies.

It's true that our interpretation is only one possible analogy from physical models. However, we establish the connection between the reduced model and the original one and explain the analogy between various physical quantities.

4.This approximation is well
known and can be very easily generalized for
non Gaussian processes (for example, for exponentially decaying correlations it
corresponds to the famous Watson lemma in expansions of Laplace
type integrals.

Thanks for pointing it out. We are aware of that.

5.would like to prove the originality and usefulness of their work, they should
make a deep comparison of their approach to huge world of Hilbert space methods
and SPDE methods in PCA analysis
of random fields.

Thanks for the suggestion. We have added the comparison and some references in the main text.

6.In addition, I should ask authors to be more accurate in description of their
numerical experiments. For example, they wrote that “the Schrödinger equation
Eq. (5) is discretized on the same grid and solved with finite difference
method.” I was puzzled: how the spectral problem (5) was solved just by finite
difference method? 

Thanks. We improved the descriptions for the numerical experiments. 

1.Under this consideration, the connection between the Gaussian field and
the Schrödinger equation is not surprising, and the efficient(near optimal)
representation of Schrödinger eigenstates have actually been used. But this
paper provided an interesting observation from general random field models, and
proposed a concrete algorithm with sample efficiency

Thanks. Indeed we are inspired by such models.

2.The general result looks convincing, while the error analysis
between PCA eigenmodes and Schrödinger eigenstates has not been established. It
would be great if the author can add a detailed analysis or provide some
criteria about the tolerance of such an approximation. 

Thanks for the question. It's hard to obtain a rigorous error estimate between the solution of approximating operators, while in practice, we use as the tolerance.

3. For applications, it is
better to explain more about the realizations of eigenmodes in these figures,
such as the meaning about different colors, directions, patterns, etc. Finally,
in the second paragraph of the Appendix A, Eq.(16)
(17) should be (A4) (A5).

Thanks for pointing out. We have addressed the typos and better illustrated the experiments.


==> response.tex <==
1.. Of course, these approximations are valid for the major
components only and become useless when the eigenfunction of (4) change
significantly on the correlation length. 

Yes, that's our setting for the model reduction.

2.This loss of validity is also obvious and unavoidable for growing index i in (4).

Not necessarily. Our method is robust even if we extract more eigenmodes, as long as the scale of the eigenmode is large so that it varies little over the correlation length.

3. Of course, a general second order elliptic equation
can be called “the Schrödinger equation”, and this analogy can help to somebody
but, at the same time, this is an elastic membrane equation, and there are many
other physically inspired analogies.

It's true that our interpretation is only one possible analogy from physical models. However, we establish the connection between the reduced model and the original one and explain the analogy between various physical quantities.

4.This approximation is well
known and can be very easily generalized for
non Gaussian processes (for example, for exponentially decaying correlations it
corresponds to the famous Watson lemma in expansions of Laplace
type integrals.

Thanks for pointing it out. We are aware of that.

5.would like to prove the originality and usefulness of their work, they should
make a deep comparison of their approach to huge world of Hilbert space methods
and SPDE methods in PCA analysis
of random fields.

Thanks for the suggestion. We have added the comparison and some references in the main text.

6.In addition, I should ask authors to be more accurate in description of their
numerical experiments. For example, they wrote that “the Schrödinger equation
Eq. (5) is discretized on the same grid and solved with finite difference
method.” I was puzzled: how the spectral problem (5) was solved just by finite
difference method? 

Thanks. We improved the descriptions for the numerical experiments. 

1.Under this consideration, the connection between the Gaussian field and
the Schrödinger equation is not surprising, and the efficient(near optimal)
representation of Schrödinger eigenstates have actually been used. But this
paper provided an interesting observation from general random field models, and
proposed a concrete algorithm with sample efficiency

Thanks. Indeed we are inspired by such models.

2.The general result looks convincing, while the error analysis
between PCA eigenmodes and Schrödinger eigenstates has not been established. It
would be great if the author can add a detailed analysis or provide some
criteria about the tolerance of such an approximation. 

Thanks for the question. It's hard to obtain a rigorous error estimate between the solution of approximating operators, while in practice, we use as the tolerance.

3. For applications, it is
better to explain more about the realizations of eigenmodes in these figures,
such as the meaning about different colors, directions, patterns, etc. Finally,
in the second paragraph of the Appendix A, Eq.(16)
(17) should be (A4) (A5).

Thanks for pointing out. We have addressed the typos and better illustrated the experiments.

